ViSNeRF: Efficient Multidimensional Neural Radiance Field Representation for Visualization Synthesis of Dynamic Volumetric Scenes

Domain scientists often face I/O and storage challenges when keeping raw data from large-scale simulations. Saving visualization images, albeit practical, is limited to preselected viewpoints, transfer functions, and simulation parameters. Recent advances in scientific visualization leverage deep learning techniques for visualization synthesis by offering effective ways to infer unseen visualizations when only image samples are given during training. However, due to the lack of 3D geometry awareness, existing methods typically require many training images and significant learning time to generate novel visualizations faithfully. To address these limitations, we propose ViSNeRF, a novel 3D-aware approach for visualization synthesis using neural radiance fields. Leveraging a multidimensional radiance field representation, ViSNeRF efficiently reconstructs visualizations of dynamic volumetric scenes from a sparse set of labeled image samples with flexible parameter exploration over transfer functions, isovalues, timesteps, or simulation parameters. Through qualitative and quantitative comparative evaluation, we demonstrate ViSNeRF's superior performance over several representative baseline methods, positioning it as the state-of-the-art solution. The code is available at https://github.com/JCBreath/ViSNeRF.

==> images/crop_info.tex <==
Loss

vortex_iso 28, 26, 195 x 185

fivejets_time_173 70, 70, 145 x 180

%%% Decoder
vortex_vol   52, 52, 150 x 152
fivejets_vol 83, 60, 138 x 123
tangaroa_vol 50, 265, 715 x 560
tangaroa_vol_zoom 95, 300, 143 x 112
tangaroa_vol_zoom 250, 310, 143 x 112 (new)

%%% Baselines
% vortex_vol 32, 32, 190 x 195
% vortex_iso 32, 29, 190 x 210
vortex_vol 40, 40, 170 x 165
vortex_iso 32, 47, 190 x 180
fivejets_vol 83, 56, 150 x 130
fivejets_iso 21, 82, 135 x 120
tangaroa_vol 226, 82, 480 x 770
% tangaroa_vol 84, 345, 740 x 445
% tangaroa_iso 171, 306, 775 x 465
tangaroa_iso 295, 143, 480 x 685
supernova_vol 164, 37, 840 x 930
supernova_iso 41, 197, 700 x 720

%%% Parameter-space Exploration
vortex_vol_tf1_030 40, 30, 185 x 185
vortex_vol_tf1_170 44, 43, 175 x 170
vortex_vol_tf2_000 57, 54, 145 x 150
vortex_vol_tf2_113 57, 57, 160 x 155
fivejets_vol_time_070 32, 74, 135, 125
fivejets_vol_time_112 80, 56, 150 x 130
tangaroa_iso_isoval_016 6, 86, 830 x 730
tangaroa_iso_isoval_134 324, 148, 440 x 545
nyx_vol_007 15, 25, 225 x 220
nyx_vol_038 30, 10, 215 x 230
nyx_vol_064 5, 5, 240 x 230
nyx_vol_096 20, 40, 195 x 190
nyx_iso_022 10, 15, 245 x 225
nyx_iso_052 10, 15, 215 x 225
nyx_iso_085 45, 25, 190 x 190
nyx_iso_164 10, 0, 240 x 235

%%% Parameter Study
fivejets_vol_iter_073 37, 72, 135 x 125
% tangaroa_iso_img_180 170, 304, 785 x 475
tangaroa_iso_img_045 222, 76, 485 x 750
supernova_vol_voxel_065 178, 59, 840 x 890
supernova_iso_sigma_064 90, 75, 720 x 840
vortex_vol_app_077 48, 39, 160 x 160
tangaroa_iso_batch_090 127, 331, 700 x 420

%%% Ablation Study
supernova_iso_split 40, 126, 700 x 760
supernova_vol_vm 32, 37, 820 x 770


%%% Upscaling
% vortex_vol_upscale_125 222, 165, 630 x 690
tangaroa_vol_upscale_180 127, 301, 825 x 480
